Self-Emotion Blended Dialogue Generation in Social Simulation Agents

When engaging in conversations, dialogue agents in a virtual simulation environment may exhibit their own emotional states that are unrelated to the immediate conversational context, a phenomenon known as self-emotion. This study explores how such self-emotion affects the agents' behaviors in dialogue strategies and decision-making within a large language model (LLM)-driven simulation framework. In a dialogue strategy prediction experiment, we analyze the dialogue strategy choices employed by agents both with and without self-emotion, comparing them to those of humans. The results show that incorporating self-emotion helps agents exhibit more human-like dialogue strategies. In an independent experiment comparing the performance of models fine-tuned on GPT-4 generated dialogue datasets, we demonstrate that self-emotion can lead to better overall naturalness and humanness. Finally, in a virtual simulation environment where agents have discussions on multiple topics, we show that self-emotion of agents can significantly influence the decision-making process of the agents, leading to approximately a 50% change in decisions.

==> figures/prompt_initiator_figure.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/prompt_initiator.pdf}
    \caption{Prompt to the probability of initiating a conversation by an agent with certain profile.}
    \label{fig:prompt_initiator}
\end{figure*}

==> figures/prompt_topic_figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/prompt_topic.pdf}
    \caption{The prompt for generating a conversation topic.}
    \label{fig:prompt_topic}
\end{figure}

==> tables/event.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{rl}
    \toprule
    \multicolumn{2}{l}{\textit{Event: grant approval}}\\
    \midrule
    \textbf{Time} & 8:00 \\
    \textbf{Labels} & excited \\
    \textbf{Duration} & 1 day \\
    \textbf{Description} & Alejandro receives a surprising\\
    & email notifying him that the \\
    & nonprofit he leads has been \\
    & approved for a significant grant. \\
    \bottomrule
    \end{tabular}
    \caption{An example of an event}
    \label{tab:event}
\end{table}

==> tables/prompt_event_table.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
    
    Given a person's profile description, generate some random events that might happen to this person in one day. The events need to: 1) be reasonable based on the description, 2) be able to affect the person's emotional status that have influence on the person's mood of that day. Each event contains 5 parts: name, description, time, emotion labels and the effective duration with each part separated with a semi-colon, ";". For emotional labels, select one most proper emotion label that this event will arise from the emotion label list used in the conversation dataset EmpatheticDialogue. The effective duration represents how long will this emotion status have influence on this person based on his/her personality. Generate at most 7 events.

    ## Example 1
    Profile: 
    Meet Alejandro Rodriguez, a passionate and community-driven 35-year-old Latino-American, originally from Mexico, making a significant impact as a Nonprofit Director in the United States. Alejandro's journey is a testament to his commitment to creating positive change and fostering community development.\n\nAlejandro, with a background in social work and public administration, has dedicated his career to addressing social issues and improving the lives of those in underserved communities. As a Nonprofit Director, he leads initiatives focused on education, healthcare, and community empowerment.\n\nHis passion for making a difference extends beyond the workplace; Alejandro actively engages with local community members, encouraging participation in various programs and fostering a sense of unity. His leadership has resulted in tangible improvements in the lives of many.\n\nOutside of his professional pursuits, Alejandro enjoys celebrating his Mexican heritage, whether through traditional music, cuisine, or community events. Alejandro Rodriguez stands as a symbol of dedication and empowerment, bridging cultural diversity for a more inclusive and vibrant community.
    Events:
    grant approval;Alejandro receives an unexpected email notifying him that the nonprofit he leads has been approved for a significant grant.;8:00;suprised;a day
    inspiring community story;Alejandro comes across the touching community letter.;11:30;grateful;1 hour
    technical glitch;The virtual presentation, with its technical issues, occurs in the early afternoon.;12:30;anxious;2 hours
    cultural celebration;Alejandro takes a break from his responsibilities and stumbles upon the impromptu cultural celebration.;13:15;trusting;1 hour
    skeptic;Toward the end of the workday, Alejandro engages in a conversation with the skeptical community member.;16:00;annoyed;45 minutes
    thank-you note;Alejandro unwinds and reads the personalized thank-you note.;18:20;joful;2 hours
    community workshop success;The success of the event becomes a satisfying way for Alejandro to wrap up the day, celebrating achievements and community engagement before heading home.;19:15;excited;3 hours
    
    ## Example 2
    Profile:
    Introducing Li Mei Chen, an ambitious and culturally connected 26-year-old Chinese-American, originally from China, thriving as a Marketing Specialist in the United States. Li Mei's journey reflects her dedication to blending her cultural roots with her professional pursuits.\n\nLi Mei, armed with a degree in marketing and international business, has quickly made a mark in the dynamic world of marketing. Her innovative ideas and cross-cultural insights have proven invaluable in crafting impactful campaigns that resonate with diverse audiences.\n\nAs a Chinese-American, Li Mei actively engages in initiatives promoting cultural understanding and connection. She is involved in community events that celebrate Chinese traditions, fostering a sense of unity and appreciation for cultural diversity.\n\nOutside the office, Li Mei enjoys practicing traditional Chinese calligraphy and exploring the rich tapestry of both her Chinese heritage and American experiences. Li Mei Chen stands as a symbol of cultural fusion, showcasing the strength that comes from embracing one's roots while navigating the possibilities of the future.
    Events:
    successful campaign launch;Li Mei begins her day with the exciting news that the marketing campaign she spearheaded has been launched successfully, receiving positive feedback from both colleagues and clients.;7:30;excited;3 hours
    unexpected recognition;Li Mei receives unexpected recognition from her supervisor for her innovative contributions to the recent campaign.;11:00;suprised;30 minutes
    cultural collaboration request;Li Mei is approached by colleagues interested in collaborating on a project that blends cultural elements into their marketing strategies.;12:45;excited;30 minutes
    cross-cultural miscommunication;Li Mei faces a challenging situation where a cross-cultural miscommunication occurs with a client.;14:00;anxious;2 hours
    networking opportunity at cultural event;Li Mei attends a cultural event in the evening, connecting with professionals from diverse backgrounds.;18:30;excited;3 hours
    
    ## Task
    Profile:
    <profile>
    Events:
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
